Open-Canopy: Towards Very High Resolution Forest Monitoring

Estimating canopy height and its changes at meter resolution from satellite imagery is a significant challenge in computer vision with critical environmental applications. However, the lack of open-access datasets at this resolution hinders the reproducibility and evaluation of models. We introduce Open-Canopy, the first open-access, country-scale benchmark for very high-resolution (1.5 m) canopy height estimation, covering over 87,000 km$^2$ across France with 1.5 m resolution satellite imagery and aerial LiDAR data. Additionally, we present Open-Canopy-$\Delta$, a benchmark for canopy height change detection between images from different years at tree level-a challenging task for current computer vision models. We evaluate state-of-the-art architectures on these benchmarks, highlighting significant challenges and opportunities for improvement. Our datasets and code are publicly available at https://github.com/fajwel/Open-Canopy.

==> figures/dynamic.tex <==
%auto-ignore
\centering
\includegraphics[width=.8\linewidth, height=.15\textheight]{example-image}

==> figures/pipeline.tex <==
%auto-ignore
\centering
\includegraphics[width=.8\linewidth, height=.15\textheight]{example-image}

==> figures/qualitative.tex <==
\centering
\begin{tabular}{c@{\,}c@{\,}c@{\,}cl}
%\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_spot_76600.jpg}
%     &  
%auto-ignore
%\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_lidar_76600.jpg}
%     &
%\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_pred_unet_76600.jpg}
%     &
%\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_pred_pvtv2_76600.jpg}
%\\
 \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_spot_80800.jpg}
    };
     \begin{scope}[x={(image.south east)},y={(image.north west)}]
     \node[fill=none, draw=none, text=black] (n1) at (0.9,0.89) {\includegraphics[width={0.025}\linewidth]{images/north.png}} ;
      \node[fill=none, draw=none, text=black] (n1) at (0.9,0.75) {\contour{white}{\scriptsize N}} ;
       \draw[-, fill=white, text=black, draw=white, ultra thick] (0.72,0.10) -- (0.93,0.10);
      \draw[<->, fill=white, text=black, draw=black,  thick] (0.70,0.10) -- (0.95,0.10);
      \draw[-, draw=black, thick] (0.825,0.10) -- (0.825,0.05);
      \node[fill=none, text=black, draw=none] at (0.825,0.18)  {\tiny  \contour{white}{\bf 250m}};
     \end{scope}
\end{tikzpicture}
     &  
\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_lidar_80800.jpg}
     &
\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_pred_unet_80800.jpg}
     &
\includegraphics[width=.225\textwidth]{images/figure_5/figure_5_pred_pvtv2_80800.jpg}
&\multirow{2}{*}[2.4cm]{
\hspace{-0.9cm}
\colorbartree{2.45cm}
}
\\
\begin{subfigure}{0.225\linewidth}
\caption{VHR image}
\label{fig:quali:a}
\end{subfigure}
&
\begin{subfigure}{0.225\linewidth}
\caption{ALS height map}
\label{fig:quali:b}
\end{subfigure}
&
\begin{subfigure}{0.225\linewidth}
\caption{UNet, MAE: %5.7 and
3.1 }
\label{fig:quali:c}
\end{subfigure}
&
\begin{subfigure}{0.225\linewidth}
\caption{PVTv2, MAE: %5.6 and
2.8 }
\label{fig:quali:d}
\end{subfigure}
\end{tabular}


==> figures/supmat_change_1.tex <==
%auto-ignore
\centering
\begin{tabular}{c@{\,}c@{\,}c@{\,}c@{\,}c@{\,}c}
\begin{subfigure}{.18\textwidth}
  \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{images/figure_supmat_change/27_spot_1.jpg}
    };
     \begin{scope}[x={(image.south east)},y={(image.north west)}]
     \node[fill=none, draw=none, text=black] (n1) at (0.145,0.89) {\includegraphics[width={0.1}\textwidth]{images/north.png}} ;
      \node[fill=none, draw=none, text=black] (n1) at (0.145,0.75) {\contour{white}{\scriptsize N}} ;
      \draw[-, fill=white, text=black, draw=white, ultra thick] (0.07,0.10) -- (0.22,0.10);
      \draw[<->, fill=white, text=black, draw=black,  thick] (0.05,0.10) -- (0.24,0.10);
      \draw[-, draw=black, thick] (0.145,0.10) -- (0.145,0.05);
      \node[fill=none, text=black, draw=none] at (0.145,0.18)  {\tiny  \contour{white}{\bf 50m}};
     \end{scope}
\end{tikzpicture}
\caption{\scriptsize VHR year 2022 }
\label{fig:supmat-change:a}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change/27_lidar_diff.jpg}
\caption{\scriptsize  ALS change map }
\label{fig:supmat-change:b}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change/27_detection_lidar.jpg}
\caption{\scriptsize ALS change mask }
\label{fig:supmat-change:d}
\end{subfigure}
\\
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change/27_spot_2.jpg}
\caption{\scriptsize VHR year 2023 }
\label{fig:supmat-change:f}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change/27_diff_pred.jpg}
\caption{\scriptsize {Our change map}  }
\label{fig:supmat-change:g}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change/27_detection_pred.jpg}
\caption{\scriptsize Our change mask}
\label{fig:supmat-change:i}
\end{subfigure}

&
\multirow[t]{2}{*}[+0.925cm]{
\hspace{-0.5cm}
\colorbargrowth{3.85cm}
}
\end{tabular}



==> figures/supmat_change_2.tex <==
%auto-ignore
\centering
\begin{tabular}{c@{\,}c@{\,}c@{\,}c@{\,}c@{\,}c}
\begin{subfigure}{.18\textwidth}
  \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{images/figure_supmat_change_2/23_spot_1.jpg}
    };
     \begin{scope}[x={(image.south east)},y={(image.north west)}]
     \node[fill=none, draw=none, text=black] (n1) at (0.145,0.89) {\includegraphics[width={0.1}\textwidth]{images/north.png}} ;
      \node[fill=none, draw=none, text=black] (n1) at (0.145,0.75) {\contour{white}{\scriptsize N}} ;
      \draw[-, fill=white, text=black, draw=white, ultra thick] (0.07,0.10) -- (0.22,0.10);
      \draw[<->, fill=white, text=black, draw=black,  thick] (0.05,0.10) -- (0.24,0.10);
      \draw[-, draw=black, thick] (0.145,0.10) -- (0.145,0.05);
      \node[fill=none, text=black, draw=none] at (0.145,0.18)  {\tiny  \contour{white}{\bf 50m}};
     \end{scope}
\end{tikzpicture}
\caption{\scriptsize VHR year 2022 }
\label{fig:supmat-change:a}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_2/23_lidar_diff.jpg}
\caption{\scriptsize  ALS change map }
\label{fig:supmat-change:b}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_2/23_detection_lidar.jpg}
\caption{\scriptsize ALS change mask }
\label{fig:supmat-change:d}
\end{subfigure}
\\
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_2/23_spot_2.jpg}
\caption{\scriptsize VHR year 2023 }
\label{fig:supmat-change:f}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_2/23_diff_pred.jpg}
\caption{\scriptsize {Our change map}  }
\label{fig:supmat-change:g}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_2/23_detection_pred.jpg}
\caption{\scriptsize Our change mask}
\label{fig:supmat-change:i}
\end{subfigure}
&
\multirow[t]{2}{*}[+0.925cm]{
\hspace{-0.5cm}
\colorbargrowth{3.85cm}
}
\end{tabular}



==> figures/supmat_change_3.tex <==
%auto-ignore
\centering
\begin{tabular}{c@{\,}c@{\,}c@{\,}c@{\,}c@{\,}c}
\begin{subfigure}{.18\textwidth}
  \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{images/figure_supmat_change_3/38_spot_1.jpg}
    };
     \begin{scope}[x={(image.south east)},y={(image.north west)}]
     \node[fill=none, draw=none, text=black] (n1) at (0.145,0.89) {\includegraphics[width={0.1}\textwidth]{images/north.png}} ;
      \node[fill=none, draw=none, text=black] (n1) at (0.145,0.75) {\contour{white}{\scriptsize N}} ;
      \draw[-, fill=white, text=black, draw=white, ultra thick] (0.07,0.10) -- (0.22,0.10);
      \draw[<->, fill=white, text=black, draw=black,  thick] (0.05,0.10) -- (0.24,0.10);
      \draw[-, draw=black, thick] (0.145,0.10) -- (0.145,0.05);
      \node[fill=none, text=black, draw=none] at (0.145,0.18)  {\tiny  \contour{white}{\bf 50m}};
     \end{scope}
\end{tikzpicture}
\caption{\scriptsize VHR year 2022 }
\label{fig:supmat-change:a}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_3/38_lidar_diff.jpg}
\caption{\scriptsize  ALS change map }
\label{fig:supmat-change:b}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_3/38_detection_lidar.jpg}
\caption{\scriptsize ALS change mask }
\label{fig:supmat-change:d}
\end{subfigure}
\\
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_3/38_spot_2.jpg}
\caption{\scriptsize VHR year 2023 }
\label{fig:supmat-change:f}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_3/38_diff_pred.jpg}
\caption{\scriptsize {Our change map}  }
\label{fig:supmat-change:g}
\end{subfigure}
&
\begin{subfigure}{.18\textwidth}
\includegraphics[width=\textwidth]{images/figure_supmat_change_3/38_detection_pred.jpg}
\caption{\scriptsize Our change mask}
\label{fig:supmat-change:i}
\end{subfigure}

&
\multirow[t]{2}{*}[+0.925cm]{
\hspace{-0.5cm}
\colorbargrowth{3.85cm}
}
\end{tabular}



==> figures/violins_bk.tex <==
%auto-ignore

==> sections/5_benchmark.tex <==
%auto-ignore






==> sections/6_discussions.tex <==
%auto-ignore

==> sections/B_checklist.tex <==
%auto-ignore
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \secref{sec:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \secref{sec:limitations}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  %auto-ignore
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The instructions to download the dataset and the code are accessible on the GitHub page given in the abstract.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \secref{sec:models}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Due to the extensive computational resources required to calculate error bars in time for the submission deadline, we were unable to include them in the current version of the paper. We plan to conduct the necessary experiments over the coming weeks and intend to incorporate error bars in the final camera-ready version of the paper, should it be accepted.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}{See \secref{sec:models}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited the source of all models and the provider of all data.}
  \item Did you mention the license of the assets?
    \answerYes{We mentioned the license of the data provider, and link to the website of all code which contains their license.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We mentioned the data provider explicitly in \secref{sec:Open-Canopy}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Datasheet for datasets in the suppmat.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
